Random Testing of Model Checkers for Timed Automata with Automated Oracle Generation

A key challenge in formal verification, particularly in Model Checking, is ensuring the correctness of the verification tools. Erroneous results on complex models can be difficult to detect, yet a high level of confidence in the outcome is expected. Indeed, these tools are frequently novel and may not have been thoroughly tested. When standard benchmarks may be insufficient or unavailable, random test case generation offers a promising approach. To scale up, random testing requires comparing actual versus expected results, i.e., solving the oracle problem. To address this challenge, this work introduces a novel theoretical framework based on a modular variant of Timed Automata (TA), called Tiled Timed Automata (TTA), for testing model checkers operating with variations of TA, by building oracles based on Weighted Automata. The framework is initially applied to verify model checkers solving the emptiness problem for Parametric TA and it is validated, in this specific scenario, by our tool, TABEC, which randomly generates tests predicting their expected outcome through automated oracle generation. Furthermore, the general nature of TTA facilitates the framework adaptation to model checkers solving other decidable problems on TA, as detailed for the minimum-cost reachability problem of Priced TA.

==> Backup_Tabella.tex <==
\definecolor{bluepoli}{cmyk}{0,0,0,0.2}
\newcolumntype{C}{>{}c}
\newcolumntype{L}{>{}l}
\begin{table}[t]
\centering 
\footnotesize
\resizebox{\textwidth}{!}{
\captionsetup{skip=5pt}
    \begin{tabular}{| L  C  C  C  C  C |}
    \hline
    \rowcolor{bluepoli} 
    \fontseries{b}\selectfont
        \textbf{Metric} & 
        \begin{tabular}{@{}c@{}}
            \textbf{\hyperref[alg:mainalgo]{EmpCheck}}
        \end{tabular} & 
        \begin{tabular}{@{}c@{}}
		    \textbf{\hyperref[alg:mainalgo]{EmpCheck}}
		\end{tabular} & 
		\begin{tabular}{@{}c@{}}      
            \textbf{EmpCheckFst}
        \end{tabular} & 
        \begin{tabular}{@{}c@{}}
            \textbf{EmpCheckFst}
        \end{tabular} & 
        \textbf{Total}\\
        \hline \hline
        \begin{tabular}{@{}l@{}}
            \#Tests
        \end{tabular} & 79 & 103 & 81 & 104 & 367\\
        \hline
        \begin{tabular}{@{}l@{}}
            MaxSize 
        \end{tabular} & 869 & 1172 & 911 & 1199 & -\\
        \hline
        \begin{tabular}{@{}l@{}}
            \#NonEmpty
        \end{tabular} & 28 & 38 & 25 & 38 & 129\\
        \hline
        \begin{tabular}{@{}l@{}}
            \#Empty
        \end{tabular} & 51 & 65 & 56 & 66 & 238\\
        \hline
        \begin{tabular}{@{}l@{}}
            Accuracy
        \end{tabular} & 100\% & 100\% & 100\% & 100\% & 100\%\\
        \hline
        \begin{tabular}{@{}l@{}}
            Timeouts[min]
        \end{tabular} & 62 & 122 & 62 & 122 & -\\
        \hline
    \end{tabular}
    }
    \caption{Scalability results of \toolname{} considering \hyperref[alg:mainalgo]{EmpCheck} and EmpCheckFst.}
    \label{table:algoscalab}
\end{table}

==> proof_backup.tex <==
\newcommand{\tile}{\mathcal{T}}
\newcommand{\acctile}{\tile_\mathit{acc}}
\newcommand{\aut}{\mathcal{A}}
\newcommand{\accset}{\mathbb{B}}
\newcommand{\pathLength}{\lvert P \rvert}
\newcommand{\patha}{P_{\mathcal{A}}}
\newcommand{\pathw}{P_{\mathcal{W}}}
\newcommand{\pathaLength}{\lvert \patha \rvert}
\newcommand{\pathwLength}{\lvert \pathw \rvert}
\newcommand{\langaut}{\mathcal{L}(\mathcal{A})}
\newcommand{\prefw}{W}
\newcommand{\outT}{w_T(\tile_0, y_1, \tile_1)}

\setcounter{theorem}{1}

\section{Proof of \autoref{thm:productivity}}
\label{app:proof_of_theorem_2}
\begin{theorem}
 {Let $\mathcal{A} = (\Theta, \mathcal{T}_{0},\Sigma, \mathbb{B}, X_{\Theta}, \Upsilon)$ be a PTTA and $\thetaWeight{}$ be a weight function as in \autoref{def:weight-of-TTA}.
   If every tile in $\Theta$ is productive for $\thetaWeight{}$, checking the non-emptiness of $\mathcal{A}$ is equivalent to checking the existence of words with non-zero weight in $\uwa{}$.
   %, the underlying weighted automaton of $\mathcal{A}$. 
   In other words, $\mathcal{L}(\mathcal{A})$ is non-empty if, and only if, 
   there exists $y \in \Sigma^*$ and a path $P$ in $\uwa{}$ with a non-zero weight in $\mathcal{B}_k$ such that $l(P) = y$.}
\end{theorem}

\begin{proof}
    
    The proof proceeds by induction over the length of paths in $\aut$ and $\uwa$ denoted, respectively, by $\patha$ and $\pathw$.
    The length of a path $\patha$, denoted by $\pathaLength$, is defined as the number of transitions traversed by $\aut$ in $\patha$.
    The length of a path $\pathw$, denoted by $\pathwLength$, is defined as the length of its label.
    Non-accepting tiles and non-accepting states can be traversed more than once.
    In the following, let
    $\patha = \tile_0\tile_1$

    (\emph{Base case}) Consider the path $\patha = \acctile$ ($\acctile \in \accset$).
    Since $\tile_\mathit{acc}$ is productive, $\langaut$ is non-empty.
    The path $\patha$ corresponds to the path $\pathw = \acctile$ ($\acctile \in F$).
    By \autoref{def:productivity}, the weight $w(\pathw)$ is non-zero and corresponds to $\delta_{\acctile}$.
    
    Conversely, consider the path $\pathw = \acctile$ ($\acctile \in F$), such that $w(\pathw)$ is non-zero.
    Since $\acctile$ is a final state in $\uwa$, the only possible corresponding path $\patha$ must contain exactly one accepting tile $\acctile \in \accset$, i.e., $\patha = \acctile$.
    Since $\acctile$ is productive, it follows that $\langaut$ is non-empty.

    Before the inductive step, we show the correspondence between intervals and weights over arbitrary paths $\patha$ and $\pathw$.
    Let $\patha = \tile_0\tile_1$, where $\tile_0 \in (\Theta \setminus \accset)$, and $\pathw = \tile_0 y_1 \tile_1$, where $\tile_0 \in (Q \setminus F)$.
    Let $\outT$ denote the weight corresponding to the parameter set of the output location where the transition from $\tile_0$ to $\tile_1$ originates in $\aut$.
    If $\tile_1 \in \accset$ over $\patha$ and $\tile_1 \in F$ over $\pathw$, then $w(\pathw) = \outT \otimes w_F(\tile_1)$ and is non-zero.
    If $\tile_1 \in (\Theta \setminus \accset)$ over $\patha$ and $\tile_1 \in (Q \setminus F)$ over $\pathw$, then $w(\pathw)$ is zero,
    still it coincides with $\outT$.

    Suppose the above correspondence holds for arbitrary paths $\patha = \tile_0 \dots \tile_{n-1}$, where $\{ \tile_0, \dots, \tile_{n-2} \} \subseteq (\Theta \setminus \accset)$, and $\pathw = \tile_0 y_1 \dots \tile_{n-1}$, where $\{ \tile_0, \dots, \tile_{n-2} \} \subseteq (Q \setminus F)$.
    We now show that it also holds for the paths $\patha' = \tile_0 \dots \tile_{n-1} \tile_n$, where $ \{ \tile_0, \dots, \tile_{n-1} \} \subseteq (\Theta \setminus \accset)$, and $\pathw' = \tile_0 y_1 \dots \tile_{n-1} y_n \tile_n$, where $ \{ \tile_0, \dots, \tile_{n-1} \} \subseteq (Q \setminus F)$.
    Let $\prefw$ be the weight of the prefix $\tile_0y_1 \dots y_{n-1}\tile_{n-1}$, computed as the product of the weights corresponding to the parameter sets of the output locations generating $\patha$, i.e., 
    $\prefw = \prod_{0 \leqslant i < n-1} w_T(\tile_{i}, y_{i+1}, \tile_{i+1})$.
    If $\tile_n \in \accset$ over $\patha'$ and $\tile_n \in F$ over $\pathw'$, then $w(\pathw') = \prefw \otimes w_T(\tile_{n-1}, y_n, \tile_n) \otimes w_F(\tile_n)$ and is non-zero.
    If $\tile_n \in (\Theta \setminus \accset)$ over $\patha'$ and $\tile_n \in (Q \setminus F)$ over $\pathw'$, then $w(\pathw')$ is zero, still it coincides with the product of $\prefw$ and the weight relative to the parameter set of the output location where the transition from $\tile_{n-1}$ to $\tile_n$ originates.

    (\emph{Inductive step}) Suppose the theorem holds for a path $\patha = \tile_0 \dots \tile_{n-1}\acctile$ ($\pathaLength = n$), where 
    $\{ \tile_0, \dots, \tile_{n-1} \} \subseteq (\Theta \setminus \accset)$ and $\acctile \in \accset$.
    The path $\patha$ corresponds to the path $\pathw = \tile_0 
    y_1
    \dots
    \tile_{n-1}
    y_{n}
    \acctile$, where 
    $\{ \tile_0, \dots, \tile_{n-1} \} \subseteq (Q \setminus F)$ and $\acctile \in F$,
    with weight
    $
    w(\pathw)= ( \prod_{0 \leqslant i < n-1} w_T(\tile_{i}, y_{i+1}, \tile_{i+1}) )
    \otimes w_T(\tile_{n - 1}, y_n, \acctile)
    \otimes w_F(\acctile)$.
    We now show that the theorem also holds for the path $\patha' = \tile_0 \dots \tile_{n-1}\tile_n\acctile$ ($\lvert \patha' \rvert = n + 1$), where $\{ \tile_0, \dots, \tile_n \} \subseteq (\Theta \setminus \accset)$ and $\acctile \in \accset$.
    Since every tile in $\Theta$ is productive, $\langaut$ is non-empty over $\patha'$.
    The path $\patha'$ corresponds to the path $\pathw' = \tile_0 
    y_1 
    \dots
    \tile_{n-1}
    y_n
    \tile_n
    y_{n + 1}
    \acctile$, where 
    $\{ \tile_0, \dots, \tile_n \} \subseteq (Q \setminus F)$ and $\acctile \in F$.
    The weight of the path $\pathw'$ is
    $
    w(\pathw')= ( \prod_{0 \leqslant i \leqslant n-1} w_T(\tile_{i}, y_{i+1}, \tile_{i+1}) )
    \otimes w_T(\tile_n, y_{n+1}, \acctile)
    \otimes w_F(\acctile)
    $.
    By the induction hypothesis, $w(\pathw)$ is non-zero.
    Since $\patha'$ is obtained by considering an additional productive tile $\tile_n$, it follows that $w(\pathw')$ is also non-zero.
    
    Conversely, suppose the theorem holds for a path $\pathw = 
    \tile_0 
    y_1 
    \dots 
    \tile_{n-1}
    y_n
    \acctile$, where $\{ \tile_0, \dots, \tile_{n-1} \} \subseteq (Q \setminus F)$ and $\acctile \in F$, having a non-zero weight $w(\pathw)$.
    Its label is $l(\pathw) = y_1 \dots y_n$ and its length is $\pathwLength = n$.
    The path $\pathw$ corresponds to the path $\patha = \tile_0 \dots \tile_{n-1}\acctile$, where $\{ \tile_0, \dots, \tile_{n-1} \} \subseteq (\Theta \setminus \accset)$ and $\acctile \in \accset$.
    We now show that the theorem also holds for the path
    $\pathw' = \tile_0 
    y_1 
    \dots 
    \tile_{n-1}
    y_n
    \tile_n
    y_{n+1}
    \acctile$ ($l(\pathw') = y_1 \dots y_{n+1}$, thus $\lvert \pathw' \rvert = n+1$), where 
    $\{ \tile_0, \dots, \tile_n \} \subseteq (Q \setminus F)$ and $\acctile \in F$, still having a non-zero weight.
    This corresponds to the path $\patha' = \tile_0 \dots \tile_{n-1}\tile_n\acctile$, where $\{ \tile_0, \dots, \tile_n \} \subseteq (\Theta \setminus \accset)$ and $\acctile \in \accset$.
    By the induction hypothesis, $\aut$ can reach $\acctile$ over the path $\patha$.
    Since the tile $\tile_n$ is productive it can be traversed by definition, thus $\aut$ can reach $\acctile$ over the path $\patha'$.
    It follows that $\langaut$ is non-empty.
    \hfill \qed
\end{proof}

==> sec-forecasting-copy/sec-forecasting-copy.tex <==
This section introduces the concepts of tiles and Tiled TA, used to generate the oracle that knows the expected parameter values of a given PnrtTA. 
\subsubsection{Tiled Timed Automata}
Tiles are particular TA that can be considered as building blocks for creating more complex TA, {having an effect which can be easily predicted}.
Tiles are defined as follows:

\begin{definition}[Tile]
    \label{def:tiledef}
    A \emph{tile} $\mathcal{T}$ is a tuple $\mathcal{T} = (\Sigma, Q, B, X, T, \mathit{In}, \mathit{Out})$, where $\Sigma$, $Q$, $B$, $X$, $T$ are as in \autoref{def:tadef} and where
    $\mathit{In} \subseteq Q$ is the set of \emph{input} locations,
    $\mathit{Out} \subseteq Q$ is the set of \emph{output} locations,
    and $B$ may be empty.
\end{definition}

%\begin{itemize}
%        \item $\mathit{In} \subseteq Q$ is the set of \emph{input} locations,
%        \item $\mathit{Out} \subseteq Q$ is the set of \emph{output} locations,
%        \item the accepting set $B$ may be empty.
%        \end{itemize}

{The \emph{language} $\mathcal{L(T)}$ of a tile $\mathcal{T}$ is the set of words accepted by the TA defined as $\mathcal{T}$.}
%\todoAM{}{Spostato sopra}
{Input and output locations are used to connect tiles together---i.e., the output location of one tile is connected to the input location of another tile.
%\Red{For simplicity, and without loss of generality, in the following we assume tiles to have only one input location.}
When needed, we use $\mathcal{T}$ as subscript to separate the elements of different tiles; for example, $\mathit{In}_{\mathcal{T}}$ and $\mathit{Out}_{\mathcal{T}}$ indicate, respectively, the input and output sets of tile $\mathcal{T}$.
If a tile $\mathcal{T}$ is such that $B_{\mathcal{T}} \neq \varnothing$, then $\mathcal{T}$ is called an \emph{accepting tile};
in that case, for all locations $q\in \mathit{In}_{\mathcal{T}}$,  
all runs from $q$ must go through an accepting location of $\mathcal{T}$.
{Transitions between different tiles are defined as follows:} 
%
%\begin{definition}
%\label{def:tilesequence}
%Given a set of $n$ tiles $\Theta = \{\mathcal{T}_{0}, \mathcal{T}_{1}, ..., \mathcal{T}_{n - 1}\}$, 
%let $\Sigma_{\Theta}=\bigcup_{\mathcal{T} \in \Theta}\Sigma_{\mathcal{T}}$ 
%and $X_{\Theta} = \bigcup_{\mathcal{T} \in \Theta}X_{\mathcal{T}}$.
%Then, tiles contained in $\Theta$ are said to be \emph{connected in sequence} iff transitions between different tiles are of the following form: $Out_{\mathcal{T}_{i}} \times In_{\mathcal{T}_{i + 1}} \times \Gamma(X_{\Theta}) \times \Sigma_{\Theta} \times 2^{X_{\Theta}}$, $\forall i \in [0, n - 2]$. 
%\end{definition}
%Therefore, when  tiles are connected in sequence if their transition graph is acyclic. 
%\todoPL{inline}{definizione alternativa:}
\begin{definition}[Tile transition relation]
    \label{def:tilesequence}
    Given an alphabet $\Sigma$ and a set of tiles $\Theta$, let 
    %    $\Sigma_{\Theta}=\bigcup_{\mathcal{T} \in \Theta}\Sigma_{\mathcal{T}}$ and 
    $X_{\Theta} = \bigcup_{\mathcal{T} \in \Theta}X_{\mathcal{T}}$ be
    %    , respectively, the alphabet and 
    the set of clocks of $\Theta$.
    A \emph{tile transition relation}  $\Upsilon$ is a set of tuples included in: 
    \begin{equation*}
    \bigcup_{\mathcal{T}, \mathcal{T}' \in \Theta} \mathit{Out}_{\mathcal{T}} \times \mathit{In}_{\mathcal{T}'} \times \Gamma(X_{\Theta}) \times \Sigma \times 2^{X_{\Theta}}.
    \end{equation*}
%\Red{A tile transition relation induces a graph, called \emph{tile transition graph}, where vertexes are tiles and edges are transitions in $\Upsilon$}. 
\end{definition}

{A tile transition relation formally defines the allowed connections between tiles, enabling the construction of arbitrarily large TA.}

\begin{definition}[Tiled TA]
    A \emph{Tiled Timed Automaton} $\mathcal{A}$ (shortened as TTA) is a tuple $\mathcal{A} = (\Theta, \mathcal{T}_{0},\Sigma, \mathbb{B}, X_{\Theta}, \Upsilon)$, where
    $\Theta$ is a set of tiles,
    $\mathcal{T}_{0} \in \Theta$ is the initial tile,
    $\Sigma$ is a finite input alphabet,
    $\mathbb{B} \subseteq \Theta$ is a set of accepting tiles,
    $X_{\Theta}$ is a set of clocks defined as: $X_{\Theta} = \bigcup_{\mathcal{T} \in \Theta} X_{\mathcal{T}}$, and
    $\Upsilon$ is a tile transition relation. %as given in \autoref{def:tilesequence}
\end{definition}

%\begin{itemize}
%        \item $\Theta$ is a set of tiles,
%        \item $\mathcal{T}_{0} \in \Theta$ is the initial tile,
%        \item $\Sigma$ is a finite input alphabet,
%        \item $\mathbb{B} \subseteq \Theta$ is a set of accepting tiles,
%        \item $X_{\Theta}$ is a set of clocks defined as: $X_{\Theta} = \bigcup_{\mathcal{T} \in \Theta} X_{\mathcal{T}}$,
%        \item $\Upsilon$ is the tile transition relation as given in \autoref{def:tilesequence}. 
%    \end{itemize}

If the input location of a tile $\mathcal{T}$ in a TTA does not have incoming transitions, then $\mathcal{T}$  is called an \emph{initial tile}, and its input location is denoted as $q_0$.
The \emph{flattening} of a TTA results in a TA obtained by substituting each tile within the TTA with its corresponding TA representation.
The $\omega$-language accepted by a TTA $\mathcal{A}$, denoted by $\mathcal{L}(\mathcal{A})$, is defined as the language accepted by the flattening of $\mathcal{A}$.
To define a B\"uchi acceptance condition \Red{for TTA, while still considering finite paths in them},
we add the condition that, if a tile is accepting, then it will force visiting at least one of its final locations infinitely often.
This guarantees that, even in the absence of cycles traversing different tiles within a given TTA, a Büchi acceptance condition can still be met.
\todoAM{}{Dire qui o dopo come si dovrebbero gestire questi cicli?}
\Red{Notice that cycles between tiles which are not accepting are still allowed.}


%\paragraph{Oracles for TTA}
\subsubsection{Oracles for TTA}
%Tile sets can be associated with a \emph{weight function} into a suitable semiring. 
%Given a set of tiles $\Theta$, the  weight function $w_{\Theta}:\Theta \to S$  associates each tile with a weight in a semiring.
\Red{A set of tiles $\Theta$ can be associated with a \emph{weight function} $w_{\Theta}:\Theta \to S$, which maps each tile to a corresponding weight in a suitable semiring.
The semiring and the corresponding weights must be manually selected for each problem at hand.}
The definition of $\omega$-language for a TTA with weights, also called \emph{Weighted TTA} (W-TTA), is the same as for TTA: the goal of weights is not to constrain the behaviors, but only to evaluate them.

Let $\mathcal{A}$ be a W-TTA. It is immediate to define a Weighted Finite State Automaton (W-FSA), denoted as $w(\mathcal{A})$, by considering the set of tiles as the set of states of the automaton and then connecting those states according to the tile transition relation of $\mathcal{A}$.
The weight of a tile becomes the weight of each transition exiting from the state corresponding to the tile. 
We call the resulting automaton $w(\mathcal{A})$
\todoAM{}{Cambiare notazione per il weighted automaton ($w()$ viene gia' usato per il weight dei path.}
the \emph{underlying weighted automaton} of $\mathcal{A}$. 
%
Weights characterize the behavior of tiles in $\mathcal{A}$ so that checking the emptiness of the flattening of $\mathcal{A}$ is equivalent to checking the emptiness of its underlying W-FSA.
\todoAM{}{Dire qualcosa di più su questa definizione?
Mettere una mini dimostrazione del corollario 1 in un'appendice?}
\begin{definition}[Productivity of the weight function]
    Given a W-TTA $\mathcal{A}$, the weight function over tiles is \emph{productive} if checking non-emptiness of $\mathcal{A}$ is equivalent to checking non-emptiness of $\uwa{}$. 
\end{definition}    

\begin{corollary}\label{thm:TTA-emptiness}
    Given a W-TTA with a productive weight function, its $\omega$-language is not empty if, and only if, there exists $y \in \Sigma^*$ such that $w_l(y)\neq 0_S$ (i.e., there is an accepting path $P$ %labeled $y$ 
with a non-zero weight in $S$ such that $l(P) = y$).
\end{corollary}

Notice that the decidability and complexity of the emptiness-checking of a Weighted Automaton depend on the chosen semiring. 
For instance, it is in polynomial-time given the min-plus semiring of \autoref{ex:semirings2}~\cite{ALMAGOR2022}:
the labels on the transitions have no  effect, and the problem reduces to finding a shortest path to an accepting state in a weighted graph. 
%\todoAM{}{Perchè non-emptiness? PL: e' lo stesso, alcuni preferiscono scrivere così}
Non-emptiness checking is also in polynomial-time for the Boolean words semiring $W^{k-\text{bit}}$  of~\autoref{ex:semirings1}, when the constant $k$ is coded in unary.  
Intuitively, given $1 \leqslant i \leqslant k$, one can replace every weight $w$ of the automaton with the weight: $w~\mathit{AND}~(0^{i-1})1(0^{k-i})$, effectively defining a finite automaton (depending on $i$). Repeating this procedure for every $i$, emptiness checking is  reduced to checking the emptiness of $k$ finite automata. 
%
The general procedure illustrating how to use W-TTA for oracle testing is reported in \autoref{alg:generalOracleTesting}.

\input{SEFMOverleaf/algorithm2}

%\paragraph{Parametric Tiled Timed Automata}
\subsubsection{Parametric Tiled Timed Automata}
Weighted tiles can be extended with the concept of parameters by adding a set $P$ of parameters to \autoref{def:tiledef}, obtaining so-called \emph{parametric tiles}. 
We only consider the case of one parameter, denoted by $\mu$. 
%\todoAM{}{Perchè possibly empty? Ho anche rimosso la descrizione dell'intervallo perchè già lo diciamo sotto}
A parametric tile can force parameter $\mu$ to be inside one or more 
%(possibly empty) 
%open 
real intervals
%having the form $(\frac{a}{2},\frac{b}{2})$, where $a \in \mathbb{N}$, $b \in (\mathbb{N}_{> 0} \cup \{+\infty\})$ and $a < b$,
%\todoMR{}{Se è "open", mi sa che dovrebbe essere $a < b$}
or to assume a single rational value.
Only parametric non-resetting test tiles with one parameter and two clocks are considered in this work (henceforth, the term \emph{tiles} will be used to denote this class of tiles).
\autoref{fig:pta12short} shows an example of such a tile.
In particular, when taking the first transition from $q_0$ to $q_1$, clock $y$ has a value equal to $\mu$.
Next, for the second transition from $q_1$ to $q_2$ to fire, clock $x$ must be equal to $\mu$ (it was reset when entering $q_1$), while clock $y$, thanks to the constraint imposed on clock $x$, must be such that $4 < y = 2\mu < 8$.
This implies that the following must hold: $2 < \mu < 4$.

\todoAM{}{Dice che non e' chiaro come mai le tile devono soddisfare la tile precondition function. Ci serve davvero definire tale funzione nel nostro lavoro?
Forse tantovale dire che le nostre tile funzionano se il clock $y$ in ingresso ha valore pari a 0.
Se togliamo la precondition function tantovale togliere anche la figura 5?}
For a tile $\mathcal{T}$ to be able to force {its} parameter value, clocks must have particular values before entering $\mathcal{T}$: 
the clock values must verify a \emph{clock precondition} $\mathcal{P}_{\mathcal{T}}(x, \alpha)$---i.e., a predicate defined \emph{ad hoc} for each tile telling which value $\alpha \in \mathbb{R}_{\geqslant 0}$ a given clock $x$ must assume.\\

\input{tilex.tex}
\input{ptta.tex}

{Given a TTA $\mathcal{A}$, we define a Parametric TTA (PTTA) as a W-TTA with the same tiles and tile transition relation of $\mathcal{A}$, and having its weight function
%(defined below)
based on the semiring $W^{k-bit}$, with $k=8C+2$, where $C$ is the maximum constant appearing in the guards of $\mathcal{A}$}.
We define the weight function as follows:
according to~\autoref{thm:parametric}, a PnrtTA can be studied by picking one or more of the following $k=8C+2$ subsets: 
%\todoPL{}{ci sono anche i valori 1/2, 1, 3/2}
$$
\{0\},
(0,\frac{1}{2}),
\{\frac{1}{2}\},
(\frac{1}{2},1),
\{1\},
(1,\frac{3}{2}),
\{\frac{3}{2}\},
(\frac{3}{2},2),
\dots,
(\frac{4C-1}{2},2C),
\{2C\},
(2C,+\infty).
$$
%
%We can associate a word in $\{0,1\}^k$ to describe any subset of the above sets. 
We can uniquely associate a word in $\{0,1\}^k$ with each choice of intervals. 
\todoAM{}{Ho rifrasato questo paragrafo spostando 'Every definition...' dopo l'esempio di figura 4}
%
%Every definition given for (Weighted) TTA (e.g., $\omega$-language, flattening) applies to PTTA as well.
%An example of PTTA is given in \autoref{fig:ptta1} (for simplicity, the weights of the tiles are not reported there).
%
Consider, for instance, the tile $\mathcal{T}$ depicted in \autoref{fig:pta12short}: the values of the parameter are in the interval $2 < \mu < 4$ to allow a path from a location in $\mathit{In}_{\mathcal{T}}$ to a location in $\mathit{Out}_{\mathcal{T}}$, and the maximum constant is $C=8$ (hence, $k = 8C + 2 = 66$); therefore, we associate the weight 
$w(\mathcal{T}) = 0^{9}1^{7}0^{k-16} \in \{0,1\}^k$ with $\mathcal{T}$.
%$00000000~11111110~00000000~00000000~00000000~00000000~0$.
%
Every definition given for (Weighted) TTA (e.g., $\omega$-language, flattening) applies to PTTA as well.

An example of PTTA is given in \autoref{fig:ptta1} (for simplicity, the weights of the tiles are not reported there).

\begin{definition}[Productivity of a tile]
Given a tile $\mathcal{T}$, we say that $\mathcal{T}$ is \emph{productive} when its language is non-empty if, and only if, the possible values of the parameter are in the set of values identified by its weight $w(\mathcal{T})$.
\end{definition}

\begin{proposition}
    If every tile in a PTTA $\mathcal{A}$ is productive, then $\Theta_{\mathcal{A}}$ is productive.
%    \todoMR{}{Il risultato mi sembra abbastanza ovvio, però lo mettiamo come "teorema"; forse, o diciamo 2 parole del tipo "it is easy to show that...", oppure lo "declassiamo" a "Proposition"?}  
\end{proposition}
\begin{corollary}\label{cor:productive-TTA}
    Given a PTTA $\mathcal{A}$ where each tile is productive, checking non-emptiness of $\mathcal{A}$ is equivalent to checking non-emptiness of $w(\mathcal{A})$.
\end{corollary}

\todoAM{}{Aggiungere qualche riga di spiegazione in piu' oppure mettere una mini dimostrazione in un'appendice?}
By analyzing separately each tile it is possible to assign a weight so that the tile is productive; this allows the application of the oracle verification procedure.

\subsubsection{Construction of arbitrary intervals}
%We introduce a special class of tiles, which are the smallest tiles which, once combined, can generate any arbitrary interval in which to force the parameter value.
%A particular class of tiles can be introduced as the smallest tiles which, once combined, can generate any arbitrary interval in which to force the parameter value.

We say that two tiles $\mathcal{T}_{1}$ and $\mathcal{T}_{2}$ are \emph{elementary} if, when connected in sequence---i.e., $\Upsilon \subseteq \mathit{Out}_{\mathcal{T}_1} \times \mathit{In}_{\mathcal{T}_2} \times \Gamma(X_{\Theta}) \times \Sigma \times 2^{X_{\Theta}} $, for $\Theta = \{\mathcal{T}_1, \mathcal{T}_2\}$, they can generate any interval in which to constrain the parameter value.
%
Notice that, since we consider PnrtTA that have at most two clocks, and given the region characterization used in~\cite{partimefor},
intervals are either punctual, or their length is a multiple of $\frac{1}{2}$.
%the finest interval granularity consists of intervals whose length is a multiple of $\frac{1}{2}$.
That is, the most general interval that can be created is either a single rational value, or it takes the form $(\frac{a}{2}, \frac{b}{2})$, where $a \in \mathbb{N}$, $b \in (\mathbb{N}_{> 0} \cup \{+\infty\})$, and $a < b$
{(closed intervals can be obtained by replacing $<$ with $\leqslant$ in the tile)}.
%
%
\todoAM{}{okkio che anche qui citiamo la clock precondition function.}
Then, the tiles of \autoref{fig:tilexample}, where $n$ is not a parameter, but a placeholder to be replaced with an integer constant to get the desired interval, are elementary, provided they satisfy the clock precondition $\mathcal{P}_{\mathcal{T}}(y, 0)$.
For example, \autoref{fig:pta12} shows a tile obtained by connecting in sequence the tiles of \autoref{fig:tileninf} (with $n = 4$) and of \autoref{fig:tile0n} (with $n = 8$).
\input{thrtile1.tex}
\input{PTTAimage.tex}

==> sec-related.tex <==
%\authortodo{Andrea}{We can put the mutation testing paper here. Also, we may delete or rephrase the part on the emptiness problem.}
%An analysis of the latest discoveries regarding decision problems for TAs, with a particular focus on the emptiness problem, was first carried out. 
%When considering traditional TAs, this decision problem is decidable in general. 
%However, when enriching TAs with parameters, i.e., real values to be determined, this problem becomes undecidable in general. 
%An exhaustive survey on the main emptiness results about different flavors of TAs is contained in \cite{etiennereach}.
%No decidability results are known in the published literature about the emptiness problem of the TA model studied in this work.\\
%Next, a survey on the most recent testing techniques and oracle classes revealed that TABEC is a random tester falling under the category of derived test oracles, i.e., oracles that make use of artifacts to build predictions on the program's output. In TABEC, the concepts of tiles and Tiled TAs (i.e., the artifacts) are used to enrich it with oracle capabilities.\\
%Finally, an investigation of available tools for working with TAs was conducted. The de-facto standard is the Uppaal tool, able to model, validate, and verify real-time systems described using the TAs formalism. However, it is not possible to express in Uppaal the emptiness problem for TAs as studied in this work. For this reason, an additional inquiry was performed, resulting in applying the tChecker tool \cite{tchecker}: this is called by TABEC to determine if the language of a given TA is empty or not.


